Optimal Energy Rationing for Prepaid Electricity Customers

For a large (and recently increasing) number of households, affordability is a major hurdle in accessing sufficient electricity and avoiding service disconnections. For such households, in-home energy rationing, i.e. the need to actively prioritize how to use a limited amount of electricity, is an everyday reality. In this paper, we consider a particularly vulnerable group of customers, namely prepaid electricity customers, who are required to pay for their electricity a-priori. With this group of customers in mind, we propose an optimization-based energy management framework to effectively use a limited budget and avoid the disruptions and fees associated with disconnections. The framework considers forecasts of future use and knowledge of appliance power ratings to help customers prioritize and limit use of low-priority loads, with the goal of extending access to their critical loads. Importantly, the proposed management system has minimal requirements in terms of in-home hardware and remote communication, lending itself well to adoption across different regions and utility programs. Our case study demonstrates that by considering both current and future electricity consumption and more effectively managing access to low-priority loads, the proposed framework increases the value provided to customers and avoids disconnections.

==> Prepaid Electricity - IEEE PowerTech - arXiv/01-intro-v3.tex <==
\section{Introduction}

Reliability in the electric power systems literature typically focuses on ensuring that the infrastructure is able to supply electricity to customers on demand. However, for many low-and-moderate income (LMI) households, a main reason for ``power outages'' is inability to pay electric bills, which may prompt service disconnections.
To avoid disconnections, LMI customers are known to ration energy use and compromise on critical needs to pay for energy - referred to as the ``heat or eat" problem \cite{bhattacharya2003heat}. A survey showed that 20\% households in the United States reduced or forwent food or medicine to pay energy costs in 2020 \cite{recs}. 
A particularly vulnerable group is customers in prepaid programs, who have to purchase credits for the energy prior to use, similar to pay-as-you-go phones. These programs are often targeted towards LMI customers, who may be enrolled either voluntarily or forcefully \cite{2022_citizensadvice}. While prepaid programs have some advantages, such as the flexibility to make multiple small payments during the month and avoiding upfront credit checks or deposits, they also present some significant disadvantages. For example, prepaid customers may pay a higher price for electricity \cite{2022_citizensadvice}. Whereas utilities are required to inform postpaid customers before a disconnection, prepaid customers can be automatically and immediately disconnected if their credit runs out. These unanticipated disconnections can be dangerous during extreme heat or cold events and for medically fragile customers. Furthermore, each disconnection-reconnection event can have a fixed charge as high as \$75 \cite{2014_liheap}. 
Despite those disadvantages, it is estimated that there are between 1 to 2.5 million prepaid electricity accounts in the United States \cite{texas_hostage_nodate}, \cite{noauthor_smart_2017} and several million in the United Kingdom \cite{2022_financialtimes}. %Prepaid electricity service is a payment model, similar to pay-as-you-go phones, where customers purchase credits for the energy prior to use. 

% Prepaid programs offer some advantages over the traditional postpaid or monthly billed programs. Customers do not need to undergo credit checks or pay a deposit and have the flexibility to make multiple small payments during the month. For the utility, prepaid accounts preclude the need for cost recovery from unpaid bills. Furthermore, prepaid programs are associated with reduction in energy usage \cite{eryilmaz2018can}.
% Unfortunately, prepaid programs also present some significant disadvantages. Prepaid customers can be automatically and immediately disconnected if their credit runs out, whereas utilities are required to inform postpaid customers before a disconnection. In some prepaid programs, each disconnection-reconnection event can have a fixed charge as high as \$75 \cite{2014_liheap} and the cost of electricity may be higher in prepaid programs \cite{oxfam}. These unanticipated disconnections can be dangerous during extreme heat or cold events and for medically fragile customers. 
\begin{comment}
Prepaid programs are targeted towards low-and-moderate income (LMI) households since they do not require deposits or credit checks. However, it is important to note that prepaid electricity service does not address the underlying problem of unaffordability of energy and is just a payment model which should not necessarily replace energy assistance programs. 
\end{comment}

%Prepaid programs are targeted towards low-and-moderate income (LMI) customers. This population is known to ration energy use and compromise on critical needs to pay for energy - referred to as the ``heat or eat" problem \cite{bhattacharya2003heat}. A survey showed that 20\% households in the country reduced or forwent food or medicine to pay energy costs in 2020 \cite{recs}. 
Considering that LMI households form a large part of the customer base of prepaid programs, many prepaid customers may not be able to refill their prepaid accounts with an amount commensurate with their desired use. This presents a need for an effective energy rationing and management framework for home appliances for this customer group, a topic that has received little attention to date. The underlying assumptions in energy rationing are significantly different from demand response, which typically assumes that changes in electricity use should be nearly invisible and non-disruptive to the customer. It is also different from typical literature on 
%A number of studies present 
home energy management systems (HEMS) \cite{beaudin2015home}, which often rely on specific in-home communication, computing, and switching hardware that may not be affordable for LMI families.
%
%Overall, only few studies on energy management explicitly account for a user-defined budget \cite{ismail2021mixed} or address the home energy management problem specifically for prepaid customers \cite{souza2020automatic}. They generate a time-based schedule for switching each appliance (load) ON/OFF. 
Aspects of prepaid electricity service have been addressed in terms of meter technology \cite{narmada2017design,gaur2014hdl}, power theft \cite{parvin2015framework}, cyber security \cite{anderson2010controls} and data management \cite{parvin2012standard}. However, only few studies explicitly account for a user-defined budget \cite{ismail2021mixed} or address the home energy management problem specifically for prepaid customers \cite{souza2020automatic}. The former study generates a time-based schedule for load actuation and switches each load ON/OFF, which may be experienced as intrusive, while the latter needs detailed information about operation time per load. %This study presents a home energy management framework for prepaid electricity customers to help manage their discretionary appliances and extend the amount of time their critical appliances are available. 


In contrast,
we present an energy rationing framework for prepaid electricity customers based on a simple threshold-based load control scheme adopted from a DC microgrid setting \cite{manur2020distributed}. Rather than directly actuating loads, %according to a detailed schedule, 
this framework \emph{enables} the use of a load by comparing the money available in the prepaid account to a monetary threshold assigned to the load. We refer to the prepaid account as the \emph{wallet} and the amount of money in the account as the \emph{wallet balance} or just \emph{balance}. If the balance is higher than the threshold, the load is enabled, i.e. it can be turned on if desired. Otherwise, it should remain off. The benefit of the proposed method is that the available budget may be more evenly spread throughout the month, and high priority loads (with lower thresholds) can be used longer. Furthermore, all loads are turned off before a disconnection occurs, thus avoiding potentially expensive disconnection-reconnection events. 

While such a threshold-based method is very easy to implement, it requires careful definition of the enabling thresholds. Thus, we formulate an optimization problem that identifies optimal threshold values while accounting for the available budget and forecasts of future electricity use. We assume that this problem is solved at regular, yet relatively infrequent intervals (e.g. daily), such that the approach lends itself well to implementation with existing 
in-home hardware and minimal remote communication.

In summary, this paper has two main contributions. First, we design an energy management framework that incorporates user-defined load priorities and helps users optimally ration their allocated energy budget across uses, while requiring minimal local computing and remote communication. This framework builds upon the control framework for prosumers in DC microgrids presented in \cite{manur2020distributed}, but extends it to (i) consider the prepaid wallet balance as a metric of available energy (ii) optimize the activation thresholds for individual loads to achieve better user satisfaction. Second, we implement our proposed method in code and demonstrate its benefit for managing household loads in a case study based on real-life energy use data obtained through the Pecan Street Dataset \cite{noauthor_dataport_nodate}.

\begin{comment}

\begin{itemize}[noitemsep]
    \item identifying the need for an energy rationing framework for prepaid customers to reduce the uncertainty of unanticipated disconnections
    \item adapting a battery storage-based control scheme for prepaid wallets 
    \item designing an energy management framework with the following features:
    \begin{itemize}[noitemsep]
        \item reduces disconnections
        \item incorporates user-defined load priorities
        \item suitable for heterogeneous settings: minimal hardware, local computing, remote communication requirements
    \end{itemize}

\end{itemize}

\end{comment}

The remaining paper is organized as follows.
Section \ref{section:model} presents the energy management framework, the optimization formulation, and comments on practical implementation. Section \ref{section:case-study} presents a case study and numerical results, while Section \ref{section:conclusion} summarizes and concludes the paper.

==> Prepaid Electricity - IEEE PowerTech - arXiv/02-model-v3.tex <==
\section{Model}
\label{section:model}
\begin{comment}
Prepaid service is shown to reduce energy usage presumably because users are more aware of their consumption in order to plan when to refill their wallets. Users may take different actions to reduce energy consumption: (1) improving efficiency by investing in better appliances and weatherization of the house (2) reducing discretionary load use e.g. TV, dish washer, (3) reducing ``critical" load use e.g. heating/cooling, refrigeration. In addition, disconnections can lead to involuntary reduction in energy consumption. LMI households may not have the disposable income to invest in more efficient appliances and weatherization, largely precluding the first option.
\end{comment}

In this section, we provide details on the model setup and the formulation of the optimal energy rationing problem. %The section ends with a discussion of some cases used for benchmarking. 
%The goal of the proposed framework is to extend the use of higher priority critical loads (such as appliances necessary for maintaining health and safety) and prevent disconnections (i.e prevent the wallet balance from going below zero which may be associated with a disconnection-reconnection fee) by compromising on the use of lower priority discretionary loads.
\begin{comment}    
Reduction in disconnections can be helpful for the utility as well since disconnection events can be associated with liability, particularly in the case of older adults, medically fragile customers, and during extreme weather events \cite{2021_nclc}.
\end{comment}


\begin{comment}
For a home energy management system (HEMS) for prepaid customers to be generalizable, it needs to be deployable in houses served by different utilities and across regions using different types of metering hardware. Therefore, the requirements from the local hardware at each house or ``local node" should be as basic as possible. The proposed framework assumes simple hardware at local nodes and a ``remote node" such as a server with better computation capabilities that computes and communicates set points to the local nodes. It assumes a communication frequency between the remote node and local nodes to be of the order of once every 24 hours and does not require high speed reliable communication infrastructure.
\end{comment}


\subsection{Threshold-based energy management}

The proposed energy rationing framework is an extension of the Self-Organizing Local Electrical Energy Network (SOLEEN), a control framework developed for DC prosumer microgrids without central control or communication \cite{manur2020distributed}. In the original SOLEEN design, each entity or household in the microgrid is assumed to have battery energy storage, with the battery state of charge representing available energy. Load control is done %using a simple threshold-based system, where each load is assigned 
by assigning each load a threshold in terms of the state of charge of the battery. If the state of charge falls below the threshold, the corresponding load is switched off. When it is above the threshold, the load is enabled, i.e. the user can decide to switch it on or off. 

Here, we adapt the SOLEEN methodology for a prepaid customer, who may not have a battery. 
Instead, we treat the prepaid wallet balance as a measure of the available energy and express load thresholds in terms of \$ (instead of state of charge) for each load. If the \$ balance falls below this threshold, the load is disabled. %An example illustrating this is shown in Figure \ref{fig:illustrative-example}. The balance in the wallet along with the threshold for a load is shown in the upper plot, the middle plot shows the so-called \textit{enable signal} for the load, and the bottom plot shows the desired power consumption and actual energy usage. The wallet is refilled three times (hours 0, 240, 480).  As the wallet balance drops below the threshold, the load is disabled and consumes no power. It is enabled when the balance is above the threshold and can be switched on to consume power.
Due to this analogy with battery energy storage, we refer to the refilling of the wallet (in \$) as a ``recharge". A major difference between a battery and a prepaid wallet is that the battery has a fixed capacity and the state of charge cannot go beyond that, whereas a prepaid wallet does not have an upper limit. Furthermore, electricity demand typically follows a diurnal pattern and the battery capacity (if recharged daily with e.g. solar PV panels) acts as a daily energy budget. In the case of a prepaid wallet, the user would not typically recharge daily. To incorporate a daily limit, we define a \emph{virtual wallet} which is different from the actual prepaid wallet, which we will refer to as the \textit{real wallet}. To match the daily pattern of electricity usage, we recharge the virtual wallet at the beginning of each day with a daily budget and compare load \$ thresholds to the virtual wallet balance. 
This setup brings in a daily budget for energy expenditure and assumes that a user would rather use a small amount of energy every day till the next recharge than use a large amount for the first few days till the wallet runs out and none for the remaining days.
%We compute the daily budget by dividing the amount corresponding to the latest recharge of the real wallet by the number of days till the next recharge\footnote{We assume that perfect information about when the real wallet will be recharged and by what amount, is available. This assumption will be addressed in future work.}. This uniformly distributes the latest recharge amount across all days till the next recharge. For example, if the real wallet is recharged on Day 1 with \$20 and the next recharge is expected on Day 11, then the daily budget with which the virtual wallet is recharged from Day 1 to 10 is \$20/10 = \$2. 
%We define thresholds in \$ and the enable signals for loads are determined by comparing the virtual wallet balance to the corresponding threshold. 
% This setup brings in a daily budget for energy expenditure and assumes that a user would rather use a small amount of energy every day till the next recharge than use a large amount for the first few days till the wallet runs out and none for the remaining days.

% \begin{figure}%[htbp]
% \centerline{\includegraphics[width = 0.4\textwidth]{images/real_wallet_load1_power.pdf}}
% \caption{\small The upper plot shows the wallet balance (in \$) and the \$ threshold, plotted against time on the x-axis. The middle plot shows the enable signal for the load, where a value of 1 indicates that the load can be turned on, and a value of 0 indicates that the load should remain off. The lower plot shows the desired power consumption (solid line) and actual energy usage (shaded). When the balance falls below the threshold, the load is turned off and the balance reduces at a slower rate.}
% \label{fig:illustrative-example}
% \end{figure}

\begin{figure}%[htbp]
\centerline{\includegraphics[width = 0.35\textwidth]{images/real_wallet_load1.pdf}}
\caption{\small Top: Wallet balance (blue) and load threshold (red) in \$. Bottom: Enable signal for the load. A value of 1 indicates that the load can be turned on, while a value of 0 indicates that the load should remain off. %When the balance falls below the threshold, the load is turned off and the balance reduces at a slower rate. 
\vspace{-5mm}}
\label{fig:illustrative-example}
\end{figure}


\subsubsection{Illustrative example} Figure \ref{fig:illustrative-example} shows an example of the proposed framework. The upper plot shows the balance in the virtual wallet along with the threshold for one of the loads, while the lower plot shows whether or not this load is enabled. %, and the bottom plot shows the desired power consumption and actual energy usage. 
In this example, the virtual wallet is refilled three times (at timestep 0, 960, 1920).  As the wallet balance drops below the threshold, the load is disabled. After this, the considered load does not consume any power and the balance of the virtual wallet reduces less quickly (other loads with a higher priority continue to consume power, such that the wallet balance continues to decrease until it reaches zero and all loads are disconnected).
Once the virtual wallet is recharged, the balance is above the threshold and the load is again enabled. % switched on to consume power.

\subsubsection{Determining control variables}
With the threshold-based control framework, there are two main control variables that need to be determined, namely (1) how the virtual wallet is recharged as a function of the real wallet balance and (2) how to choose thresholds for effective energy rationing. 
To determine the daily virtual wallet recharge, we simply divide the most recent recharge amount for the real wallet by the number of days until the next recharge\footnote{We assume perfect information about when and what amount will be added to the real wallet. The effect of imperfect real recharge information may be addressed by more sophisticated daily virtual wallet recharge schemes, such as allocating a variable daily budget based on the fraction of the average real recharge per month that has been spent. This is a part of future work.}. This uniformly distributes the latest recharge amount across all days till the next recharge. 
The process for determining the load enable thresholds is more sophisticated. These thresholds are obtained by solving an optimization problem as discussed below.


\begin{comment}
    
\begin{figure}[htbp]
\centerline{\includegraphics[width = 0.4\textwidth]{images/real_virtual_plot.pdf}}
\caption{\small The top figure shows the real wallet balance for a month in a scenario when the customer recharges the wallet three times and no electricity is used. The bottom plot shows the how the real wallet recharges translate to the virtual wallet being recharged daily.}
\label{fig:real_virtual_plot}
\end{figure}

\end{comment}


% \subsubsection{Implementation through a prepaid program}
% A benefit of the proposed framework is that it requires minimal additional hardware, computation and remote communication.

% \noindent\emph{A) Computational requirements:} Prepaid programs generally install in-home displays in the customer's house that show their wallet balance \cite{noauthor_srp_nodate}. 
% %For the proposed framework to directly actuate loads in a user's home, additional hardware such as smart switches is necessary. In some cases, users may not be able to afford this additional hardware or may not be comfortable with an application directly controlling certain household appliances such as medical equipment. For such users, we propose sending notifications or ``nudges" via the in-home display when the load enable signal is zero to suggest to the user that they switch off the load to ensure that loads higher up in the priority order can remain on longer. 
% The in-home display is connected to the meter and computes and displays the real wallet balance in real-time. It can be programmed to keep track of the virtual wallet as well, and since this is a simple algebraic operation, additional computation hardware is not be necessary. 

% \noindent\emph{B) Communication requirements:} Households that struggle to pay energy bills may also fall behind on internet and phone bills, thus limiting options for communication. The optimized thresholds can be computed on a remote server and communicated to the in-home display at the beginning of each day through the same communication channel that the utility uses to connect to the in-home display (e.g. the Advanced Metering Infrastructure (AMI) communication system). Since thresholds need to be communicated only once a day, communication delays can be tolerated. 

% \noindent\emph{C) Hardware requirements:} Direct actuation of loads in a user's home requires additional hardware such as smart switches. If users cannot afford this additional hardware or are not comfortable with an application directly controlling certain household appliances such as medical equipment,
% either the in-home display or a phone application can instead provide ``nudges'' to suggest to the user that they switch off the load to allow them to use higher priority loads later on.

%It follows that the proposed framework lends itself well to implementation using the existing infrastructure and may not need significant technological overheads. 
%Real-world implementation may of course present additional hurdles in terms of logistics and user acceptance. The framework can be offered on a pilot basis to evaluate the ratio of benefits to overheads.

\vspace{-1.3mm}
\subsection{Optimization formulation}
\label{section:optimization-formulation}
The optimization model determines thresholds for each load $k$ at time $t$ denoted by $\mathbf{x_{k,t}}$. The thresholds for each load are kept constant throughout each day, so the number of unique thresholds is equal to the number of loads times the number of days in the optimization horizon. The input parameters include user-defined priority order for loads, demand forecast, and recharge schedule forecast. We implement the model as a rolling horizon problem with a forecast horizon of seven days and a time step of 15 minutes. We solve the problem once daily, then use the optimized thresholds for the first day to simulate the use of loads to calculate the resulting real and virtual wallet balances. These balances, along with updated forecasts, are used as an input when we re-solve the optimization problem the next day. 
%With both on/off variables used represent the status of a load and the continuous wallet balances, t
The resulting optimization problem is a mixed-integer linear programming problem.
%We use a horizon of seven days and the duration of each time step is 15 minutes, which gives 96 time steps per day. 
The nomenclature is given in Table \ref{tab:nomenclature}. 

\begin{table}[]
    \centering    
    \caption{Nomenclature}
    \begin{tabular}{ll}
        \multicolumn{2}{l}{\textbf{Parameters}}\\
        $\mathcal{K}$ & Set of all loads\\
$\mathcal{T}$ & Set of all time steps in the horizon\\
$\Delta T \in \mathbb{R}_{> 0}$ & Duration of time step in  hours\\
$m \in \mathbb{R}_{<0}$ & Large magnitude constant \\
$M \in \mathbb{R}_{>0}$ & Large magnitude constant\\
$\epsilon \in \mathbb{R}_{>0}$ & Small magnitude constant \\
$\alpha \in \mathbb{R}_{>0}$ & Electricity rate in \$/Wh\\
$\gamma_k \in \mathbb{R}_{>0}$ & Priority factor for load $k$ \\
$P_{k,t} \in \mathbb{R}_{\geq 0}$ & Demand in W for load $k$ at time $t$, \\
$d_{k,t} \in \{0,1\}$ & Indicator parameter of demand \\
& $d_{k,t} = 1$ if $P_{k,t} > 0$, and $0$ otherwise\\
$Z_t \in \mathbb{R}_{\geq 0}$ & Real wallet recharge at time $t$ in \$\\
$X_t \in \mathbb{R}_{\geq 0}$ & Virtual wallet recharge at time $t$ in \$ \\[+3pt]
        \multicolumn{2}{l}{\textbf{Variables}}\\
        $\mathbf{z_t} \in \mathbb{R}$ & Real wallet balance at time $t$\\
$\mathbf{u^z_{k,t}} \in \{0,1\}$ & Real enable signal for load $k$ at time $t$\\
$\mathbf{x_t} \in \mathbb{R}$ & Virtual wallet balance at time $t$\\
$\mathbf{x_{k,t}} \in \mathbb{R}$ & Threshold for load $k$ at time $t$\\
$\mathbf{u^x_{k,t}} \in \{0,1\}$ & Virtual enable signal for load $k$ at time $t$ \\ 
$\mathbf{a_{k,t}} \in \{0,1\}$ & Actuation state of load $k$ at time $t$
    \end{tabular}
    \label{tab:nomenclature}
\vspace{-4mm}
\end{table}


% \noindent
% \textbf{Parameters}\\
% $\mathcal{K}$ : set of all loads\\
% $\mathcal{T}$ : set of all time steps in the horizon\\\
% $\Delta T \in \mathbb{R}_{> 0}$ : duration of time step in  hours\\
% $m \in \mathbb{R}_{<0}$, $M \in \mathbb{R}_{>0}$ : large magnitude constants for enable signal constraints\\
% $\epsilon \in \mathbb{R}_{>0}$ : small constant for enable signal constraints\\
% $\alpha \in \mathbb{R}_{>0}$ : electricity rate in \$/Wh\\
% $\gamma_k \in \mathbb{R}_{>0}$ : priority factor for load $k$ \\
% $P_{k,t} \in \mathbb{R}_{\geq 0}$ : demand in W for load $k$ at time $t$, \\
% $d_{k,t} \in \{0,1\}$ : indicator of demand for load $k$ at time $t$,  $d_{k,t} = 1$ if $P_{k,t} > 0$, and $0$ otherwise\\
% $Z_t \in \mathbb{R}_{\geq 0}$ : real wallet recharge at time $t$ in \$\\
% $X_t \in \mathbb{R}_{\geq 0}$ : virtual wallet recharge at time $t$ in \$\\
% \textbf{Variables}\\
% $\mathbf{z_t} \in \mathbb{R}$ : real wallet balance at time $t$\\
% $\mathbf{u^z_{k,t}} \in \{0,1\}$ : real enable signal for load $k$ at time $t$\\
% $\mathbf{x_t} \in \mathbb{R}$ : virtual wallet balance at time $t$\\
% $\mathbf{x_{k,t}} \in \mathbb{R}$ : threshold for load $k$ at time $t$\\
% $\mathbf{u^x_{k,t}} \in \{0,1\}$ : virtual enable signal for load $k$ at time $t$ \\ 
% $\mathbf{a_{k,t}} \in \{0,1\}$ : actuation state of load $k$ at time $t$\\


\subsubsection{Real wallet constraints}
%We first describe the constraints which express the amount of money in the real wallet as well as constraints that ensure that all loads are turned off if the real wallet balance falls below zero. 
The amount of money in the real wallet gets updated according to the energy consumption in the previous time step and the recharge amount scheduled for the current time step as given by
\begin{equation}
    \mathbf{z_{t}} = \mathbf{z_{t-1}} + Z_t - \alpha\Delta T \sum_{k\in\mathcal{K}}(P_{k,t-1}\mathbf{a_{k,t-1}}) \quad \forall t \in \mathcal{T}
\label{eq:real-recharge}
\end{equation}
\vspace{-1mm}
%(\ref{eq:real-recharge}). 
Here, $Z_t$ is equal to the recharge scheduled for the day (if any) if $t$ is the first time step of the day and zero otherwise. %Constraints (\ref{eq:real-enable}) and (\ref{eq:real-disable}) respectively 
The real enable signal $\mathbf{u^z_{k,t}}$ expresses whether there is money in the real wallet. If the real wallet balance $\mathbf{z_t}$ is positive, $\mathbf{u^z_{k,t}}=1$, and otherwise is zero. This is enforced by
%\begin{align}
% \begin{equation}
% \mathbf{z_{t}} = \mathbf{z_{t-1}} + Z_t - \alpha\Delta T \sum_{k}(P_{k,t-1}\mathbf{a_{k,t-1}}) \quad \forall t \in \mathcal{T}
% \label{eq:real-recharge}
% \end{equation}
\begin{align}
    m\mathbf{u^z_{k,t}}&\leq -\mathbf{z_t} \quad &&\forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:real-enable}\\
%\end{equation}
%\begin{equation}
    (M+\epsilon)(1-\mathbf{u^z_{k,t}})&\geq \epsilon - \mathbf{z_t} \quad &&\forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:real-disable}
%\end{equation}
\end{align}

\subsubsection{Virtual wallet constraints}
%Similar to the real wallet balance, t
The virtual wallet balance $\mathbf{x_t}$ is updated according to the energy consumption since the previous time step and the daily virtual recharge $X_t$ computed from the real recharge, i.e.
\begin{equation}
    \mathbf{x_t} = \mathbf{x_{t-1}} + X_t - \alpha\Delta T\sum_{k}(P_{k,t-1}\mathbf{a_{k,t-1}}) \quad \forall t \in \mathcal{T}
    \label{eq:virtual-recharge}
\end{equation}
%This is given by (\ref{eq:virtual-recharge}).
where $X_t$ is equal to the recharge scheduled for the day if $t$ is the first time step of the day and zero otherwise. %Constraints (\ref{eq:virtual-enable}) and (\ref{eq:virtual-disable}) respectively 
The virtual enable signal $\mathbf{u^x_{k,t}} \in \{0,1\}$ %, associated with the state of the virtual wallet $\mathbf{x_t}$ for each load $k$, 
should be 1 if the virtual wallet balance $\mathbf{x_t}$  is greater than or equal to the load threshold $\mathbf{x_{k,t}}$, or otherwise zero, as expressed by
\begin{align}
    \mathbf{x_t} - \mathbf{x_{k,t}} + \epsilon &\leq (M+\epsilon)\mathbf{u^x_{k,t}} \quad &&\forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:virtual-enable}\\
    \mathbf{x_t} - \mathbf{x_{k,t}} &\geq m(1-\mathbf{u^x_{k,t}}) \quad &&\forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:virtual-disable}
\end{align}
Note that $\mathbf{x_{k,t}}$ is also constrained to be the same for all time steps $t$ during a single day.

% \begin{equation}
%     \mathbf{x_t} = \mathbf{x_{t-1}} + X_t - \alpha\Delta T\sum_{k}(P_{k,t-1}\mathbf{a_{k,t-1}}) \quad \forall t \in \mathcal{T}
%     \label{eq:virtual-recharge}
% \end{equation}
% \begin{equation}
%     \mathbf{x_t} - \mathbf{x_{k,t}} + \epsilon \leq (M+\epsilon)\mathbf{u^x_{k,t}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
%     \label{eq:virtual-enable}
% \end{equation}
% \begin{equation}
%     \mathbf{x_t} - \mathbf{x_{k,t}} \geq m(1-\mathbf{u^x_{k,t}}) \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
%     \label{eq:virtual-disable}
% \end{equation}

\subsubsection{Actuation constraints}
The actuation constraints describe whether a load is on and consuming power. 
The actuation state $\mathbf{a_{k,t}}$ of load $k$ at time $t$ is zero if there is no demand $d_{k,t}$, the virtual wallet balance $\mathbf{x_t}$ is less than its threshold $\mathbf{x_{k,t}}$, if the real wallet balance $\mathbf{z_t}$ is less than or equal to zero, or if the real wallet balance in the next time step $\mathbf{z_{t+1}}$ would be less than or equal to zero if the load is kept on (the latter condition ensures that the real wallet balance does not go negative by the next time step). In this case, $\mathbf{a_{k,t}}=0$ as expressed by the following constraints
\begin{equation}
    \mathbf{a_{k,t}}\!\leq\! d_{k,t}\mathbf{u^x_{k,t}}, ~~ \mathbf{a_{k,t}}\!\leq\!\mathbf{u^z_{k,t}}, ~~ \mathbf{a_{k,t}} \!\leq\!\mathbf{u^z_{k,t+1}} ~~\forall k\!\in\!\mathcal{K}, \forall t\!\in\!\mathcal{T} \nonumber
    %\label{eq:actuation-1}
\end{equation}
If none of the above conditions are satisfied, the actuation state has to be equal to 1, i.e. $\mathbf{a_{k,t}}=1$, as described by % (constraint (\ref{eq:actuation-on}).
%
\begin{comment}
\begin{equation}
    \mathbf{a_{k,t}} \leq d_{k,t}\mathbf{u^x_{k,t}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:actuation-demand-virtualenable}
\end{equation}
\begin{equation}
    \mathbf{a_{k,t}} \leq \mathbf{u^z_{k,t}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:actuation-realenable-t}
\end{equation}
\begin{equation}
    \mathbf{a_{k,t}} \leq \mathbf{u^z_{k,t+1}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:actuation-realenable-tp1}
\end{equation}
\end{comment}
% \begin{equation}
%     \mathbf{a_{k,t}} \leq d_{k,t}\mathbf{u^x_{k,t}},  \mathbf{u^z_{k,t}}, \mathbf{u^z_{k,t+1}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
%     \label{eq:actuation-1}
% \end{equation}
\begin{equation}
    d_{k,t}\mathbf{u^x_{k,t}} + \mathbf{u^z_{k,t}} + \mathbf{u^z_{k,t+1}} \leq 2 + \mathbf{a_{k,t}} \quad \forall k \in \mathcal{K}, \forall t \in \mathcal{T}
    \label{eq:actuation-on}
\end{equation}
% The above constraints are a way of expressing $\mathbf{a_{k,t}} = d_{k,t}\mathbf{u^z_{k,t}}\mathbf{u^z_{k,t+1}}\mathbf{u^x_{k,t}} = d_{k,t}\mathbf{u_{k,t}}$ in terms of linear constraints, where $\mathbf{u_{k,t}} = \mathbf{u^z_{k,t}}\mathbf{u^z_{k,t+1}}\mathbf{u^x_{k,t}}$, can be interpreted as the combined enable signal.


\subsubsection{Objective function}
Our goal is to maximize the value provided to the customer from using a limited (less than desired) amount of electricity. 
To express this, we make a few key assumptions.
%We wish to maximize the value that a user obtains from using loads. 
First, some loads bring more value, i.e. 
have a higher priority, as compared to others and the value of a load does
not necessarily scale with its power rating. For instance, a light bulb rated at 5W can provide more value than a TV rated at 100W. Second, we assume that value is associated with whether or not a load is available when desired. Therefore, we design our objective function to account for (1) the priority assigned to each load by the user and (2) the percentage of time the load was available when desired. %We now present our choice of the objective function that accounts for these factors. 

We introduce the \emph{load priority factor} $\gamma_k$ to express the relative value of satisfying the demand of load $k$ compared to other loads. It is calculated as $\gamma_k = \frac{1}{\eta_k}\frac{1}{\sum\limits_k \frac{1}{\eta_k}}$, where $\eta_k$ is a number that represents the position of the load in the priority order (lower numbers imply higher priority). For example, if the user ranks loads k = 1, 2, 3 in the order 2, 3, 1 then $\eta_1 = 2$, $\eta_2 = 3$, $\eta_3 = 1$. Note that this is not the only way to determine load priority factor, and this was chosen since it ensures that $\sum_k \gamma_k = 1$. 

Next, we define the \emph{Service Factor} ($SF_k$) for each load $k$ as the ratio of the amount of time a load was available to the amount of time it was demanded.
\begin{equation}
    %SF_k = \frac{\sum\limits_t \mathbf{a_{k,t}}}{\sum\limits_t d_{k,t}}
    SF_k = {\sum\limits_t \mathbf{a_{k,t}}}~{\huge /}~{\sum\limits_t d_{k,t}}
    \label{eq:service-factor-definition}
\end{equation}
The service factor expresses the percentage of time the load was available when desired and is independent of the power rating of the load. For example, a light rated at 5W demanded for 6 hours and served for 3 hours will have the same service factor as a TV rated at 100W demanded for 2 hours and served for 1 hour. Both will have $SF_k = 0.5$. 

%A weighted average of service factors using the load priority factor accounts for the three requirements identified above. We denote this as t
The \emph{Priority Service Factor} (PSF) is the weighted average of the service factors, where the weight is the load priority factor. Our objective is to maximize the PSF, 
\begin{equation}
    \max~~ \sum_{k\in\mathcal{K}}\gamma_{k}SF_k
    \label{eq:psf}
\end{equation}
%This can also be interpreted as a multi-objective optimization problem where the objective function is expressed as a convex combination of the service factor $SF_k$ for each load $k$. %The PSF is defined as: 

\begin{comment}
\begin{equation}
    PSF = \sum_{k}\gamma_{k}\frac{\sum\limits_t \mathbf{\mathbf{a_{k,t}}}}{\sum\limits_t d_{k,t}}
    \label{eq:psf}
\end{equation}
\end{comment}


\subsection{Benchmark Cases}
To compare the proposed method, we also implement a simulation of two benchmark cases:
\subsubsection{Baseline} The baseline case does not have any energy manager and assumes that all loads are enabled as long as the real wallet balance is positive (i.e., it is a greedy approach). From a mathematical perspective, this formulation only considers the real wallet update \eqref{eq:real-recharge} and sets $\mathbf{a_{k,t}}=1$ if $d_{k,t}=\mathbf{u_{k,t}^z}=1$. 
\subsubsection{Fixed Thresholds} The fixed thresholds case uses a similar model as the one described in Section \ref{section:optimization-formulation}, except that the load thresholds $\mathbf{x_{k,t}}$ are fixed (i.e., not optimized). While there could be many methods for computing these fixed thresholds, we choose to calculate them once at the beginning of the month as 
$\mathbf{x_{k,t}} = \frac{\eta_k}{N} \beta X \quad \forall t$.
Here, $\eta_k$ is the position of Load $k$ in the priority order, $N$ is the total number of loads, $X$ is the total recharge amount for the month (in \$), and $\beta$ is a positive constant less than 1. For this study, $\beta = 0.05$ was used. With this definition, lower priority loads (i.e. those with a higher $\eta_k$) are assigned higher thresholds and will get disabled before higher priority loads as the wallet balance drops. %The fixed thresholds case always has residual balance equal to at least the lowest threshold i.e. the threshold corresponding to the highest priority load.

\subsection{Implementation through a prepaid program}
A benefit of the proposed framework is that it requires minimal additional hardware, computation and remote communication, and thus lends itself well to implementation using the existing infrastructure without significant technological overheads. 

\noindent\emph{A) Computational requirements:} Prepaid programs generally install in-home displays in the customer's house that show their wallet balance \cite{noauthor_srp_nodate}. 
%For the proposed framework to directly actuate loads in a user's home, additional hardware such as smart switches is necessary. In some cases, users may not be able to afford this additional hardware or may not be comfortable with an application directly controlling certain household appliances such as medical equipment. For such users, we propose sending notifications or ``nudges" via the in-home display when the load enable signal is zero to suggest to the user that they switch off the load to ensure that loads higher up in the priority order can remain on longer. 
The in-home display is connected to the meter and computes and displays the real wallet balance in real-time. It can be programmed to keep track of the virtual wallet as well, and since this is a simple algebraic operation, additional computation hardware may not be necessary. 

\noindent\emph{B) Communication requirements:} Households that struggle to pay energy bills may also fall behind on internet and phone bills, thus limiting options for communication. The optimized thresholds can be computed on a remote server and communicated to the in-home display at the beginning of each day through the same communication channel that the utility uses to connect to the in-home display (e.g. the Advanced Metering Infrastructure (AMI) communication system). Since thresholds need to be communicated only once a day, communication delays can be tolerated. 

\noindent\emph{C) Hardware requirements:} Direct actuation of loads in a user's home requires additional hardware such as smart switches. If users cannot afford this additional hardware or are not comfortable with an application directly controlling certain household appliances such as medical equipment,
either the in-home display or a phone application can instead provide ``nudges'' to suggest to the user that they switch off the load to allow them to use higher priority loads later on.


\begin{comment}
It is important to note that a user who may be struggling to recharge their prepaid wallet in time may also be behind on their internet and phone bills. The utility uses communication channels such as power-line, cellular, or radio frequency which are independent of the user's cellular or internet connection to communicate with the meter \cite{VANDEKAA2019320}. Therefore, the same channels can be used to communicate the thresholds. 


It follows that the proposed framework lends itself well to implementation with the existing infrastructure without significant technological overheads. Real-world implementation may present additional hurdles in terms of logistics, customer acceptance, and user experience. For example, a user needs to provide the priorities assigned to each appliance and measurements have to be made to obtain their power ratings. Since there are numerous appliances, some appliances can be lumped together, for instance all kitchen appliances can be lumped together as kitchen load and be assigned a single priority. Furthermore, to forecast demand with appliance-level granularity, load disaggregation may be necessary. The utility can offer the framework on a pilot basis and evaluate the ratio of benefits to overheads before large scale deployment.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> Prepaid Electricity - IEEE PowerTech - arXiv/03-case-study.tex <==
\section{Case study}
\label{section:case-study}
We next demonstrate our proposed framework for optimal energy rationing with a case study. We compare the proposed optimal method against the two benchmark cases, and assess the impact of recharge frequency and overall recharge amount on the priority service factor and the number of disconnections.

\begin{figure}%[htbp]
\centerline{\includegraphics[width = \columnwidth]{images/load_power_plot.pdf}}
\vspace{-2mm}
\caption{Load power demand for 30 days (W).}
\label{fig:load_power_plot}
\end{figure}
\vspace{-3mm}
\begin{table}%[htbp]
\caption{Load data\vspace{-3mm}}
\begin{center}
\begin{tabular}{m{2em} m{7em} m{3em} m{5em} m{3.5em}}
\hline
\multicolumn{2}{l}{\textbf{Appliance}} & \textbf{Energy (kWh)} & \textbf{Max Power (kW)} & \textbf{Load Priority}\\
\hline
A & air compressor & 28 & 1.9 & 2\\ 
B & washing machine  & 2.0 & 0.44 & 4\\
C & microwave & 3.6 & 1.2 & 3\\
D & refrigerator & 41 & 0.38 & 1\\
\hline
\end{tabular}
\vspace{-5mm}
\label{tab:load-data}
\end{center}
\end{table}
\subsection{Setup and implementation}
%\subsubsection{Data and parameters}
%The case study uses 
We use load data for one month (30 days) from one house in the Pecan Street Dataset \cite{noauthor_dataport_nodate}. The four loads used are an air compressor (Load A), a washing machine (Load B), a microwave (Load C), a refrigerator (Load D). Figure \ref{fig:load_power_plot} shows the power demand for each load for the duration of the month and Table \ref{tab:load-data} summarizes the total energy demand, maximum power demand, and priority for each load.




%\subsubsection{Parameters}
%For this case study, 
We assume that perfect information about the current and future demand for each load as well as the recharge amount and timing is available to the model. (Considering effects of imperfect information and user non-compliance are a part of future work and may be addressed through more sophisticated schemes such as variable daily virtual wallet recharge.) The presented results assume either direct load actuation through smart switches or total user compliance to the load enable signal nudges given by the model, i.e. we assume that a load is only in use when the corresponding load actuation signal is $\mathbf{a_{k,t}=1}$. We use an electricity rate of $\alpha = \text{\$}0.15/kWh$. Since this is a parameter, time-of-use pricing (i.e. time-varying $\alpha(t)$) may be incorporated without changing the complexity of the problem. The total cost of electricity for using the devices in Table \ref{tab:load-data} with a constant $\alpha = \text{\$}0.15/kWh$ would thus be \$11.19 \footnote{ Additionally, a transaction cost (fee associated with each recharge) and a monthly fixed cost can be included and is considered part of future work. Factors such as whether the fixed cost will be deducted from the wallet per day or upfront at the beginning of the month may influence model performance.}.


The \emph{recharge frequency} is the number of times a user recharges their wallet in a month, and typically varies between 1 and 7 per month \cite{2010_epri}. We express the total recharge as the fraction of the total cost of desired electricity. The \emph{recharge amount} is the total amount of money added to the real wallet over the course of the month. We express this amount as a percentage of the amount needed to cover the desired electricity use listed in Table \ref{tab:load-data}. Thus, recharge amounts $<100$\% imply a need for rationing. % Since this recharge amount may not be sufficient to cover the total cost of electricity that the household would ideally like to use (i.e., it may be less than \$11.19). 
We assume that the total recharge amount is uniformly distributed across all recharges.


The proposed optimization model and the benchmarking cases are implemented in the Julia programming language \cite{bezanson2017julia} (v1.6) and run on a machine with an Intel CPU @3.2GHz and 16GB memory. In the optimized thresholds case, the simulation calls the optimization model implemented using JuMP \cite{dunning2017jump} and the Gurobi solver \cite{gurobi}. The parameter $\epsilon$ was set to 1e-6 which is equal to the default tolerance of the solver Gurobi to meet constraints. %once per day and obtains thresholds for the day.
The optimization model computes new thresholds daily, using an optimization horizon of 7 days. The thresholds for the current day are then implemented in the simulation. The real and virtual wallet balances at the end of the simulated day are then used as an input for the optimization problem the next day.

%We present results by variation of two parameters, the monthly recharge frequency and the total recharge amount. The monthly recharge frequency is the number of times a user recharges their wallet in a month. The recharge frequency can be as high as 7 per month in summer \cite{2010_epri}. The total amount added to the wallet by an LMI household in the month may not be equal to the total cost of electricity that they would ideally like to use. The total recharge amount is therefore expressed as the fraction of this total cost of desired electricity. It is assumed that the total recharge amount is uniformly distributed across all recharges.


% \subsubsection{Cases}
% We compare results for three different cases:\\
% \paragraph{Baseline} The baseline case does not have any energy manager and assumes that all loads are enabled as long as the real wallet balance is positive. \\
% %For this case, the household experiences a disconnection if the real wallet balance goes below zero.\\
% \emph{Optimized thresholds} The optimized thresholds case implements the model described in Section \ref{section:optimization-formulation} to determine the load thresholds $\mathbf{x_{k,t}}$ that will be used to generate load enable signals.\\
% \emph{Fixed thresholds} The fixed thresholds case uses thresholds on the virtual wallet that are computed once at the beginning of the month as follows: $x_{k,t} = \frac{\eta_k}{N} \beta X \quad \forall t$, where $\eta_k$ is the position of Load $k$ in the priority order, $N$ is the total number of loads, $X$ is the total recharge amount for the month (in \$), and $\beta$ is a positive constant less than 1. For this study, $\beta = 0.05$ was used. With this defintion, a lower priority load (i.e one with a higher $\eta_k$) is assigned a higher threshold and will get disabled before a higher priority load as the wallet balance drops.
% \begin{comment}
% \begin{equation}
%     x_{k,d} =  \frac{\eta_k}{N} \beta X \quad \forall d
%     \label{eq:fixed-threshold}
% \end{equation}
% \end{comment}


% \subsubsection{Metrics}
% Results are compared using the following metrics.
% \begin{itemize}
%     \item Service Factor ($SF_k$) per load as defined by (\ref{eq:service-factor-definition}).
%     \item Priority Service Factor (PSF) for the overall set of loads as defined by (\ref{eq:psf}).
%     \item Number of disconnections: A disconnection is defined as an event when the real wallet goes negative.
% \end{itemize}

%\paragraph{Energy Service Factor (ESF)} The ESF represents the percentage of total energy demand served across all loads over the duration of the simulation.
%\begin{equation}
%    ESF = \frac{\sum_{k,t} a_{k,t}P_{k,t}}{\sum_{k,t} d_{k,t}P_{k,t}}
%\end{equation}

% \subsubsection{Implementation}
% The three cases are implemented in the Julia programming language \cite{bezanson2017julia} (v1.6) on a machine with an Intel CPU @3.2GHz and 16GB memory. In the optimized thresholds case, the simulation calls the optimization model implemented using JuMP \cite{dunning2017jump} and the Gurobi solver \cite{gurobi} once per day and obtains thresholds for the day.

\begin{comment}

As an additional protection layer against disconnections, the fixed and optimized thresholds cases have a local override signal implemented in the simulation. If the actuation state of loads at time $t$, as determined by comparing the current virtual wallet balance with the thresholds for the day, is found to lead to a negative real wallet balance at time $t+1$ due to numerical discrepancies between the model and the simulation, the local override signal disables all loads at time step $t$. Even though all loads are curtailed, this avoids a disconnection-reconnection event which may entail high charges.
\end{comment}

%\subsection{Numerical Results}
%\subsubsection{Service factor}
\subsection{Comparison with Benchmark Cases}
As a first investigation, we compare the performance of the optimal energy rationing framework with the baseline and fixed thresholds benchmark cases. To do this, we run each method for the full 30 days and compare the resulting service factors (SF) per load as defined by \eqref{eq:service-factor-definition}, the overall achieved priority service factor (PSF) as defined by \eqref{eq:psf}, as well as the amount of energy consumed per load. For this evaluation, we assume a recharge amount of 70\% and a recharge frequency of 5 payments per month.
Figure \ref{fig:recharge70realrf5load_tsf_psf_barchart} shows the service factor $SF_k$ for each load and the overall PSF and Table \ref{tab:energy-use-per-load} shows the energy use per load. We observe that the different cases lead to very different use of energy across the different loads. The refrigerator (Load D) has the highest priority, and is also the load that runs most continuously. The optimized and fixed threshold cases achieve both a service factor and energy use close to 100\% for this load, while the baseline case (which experiences a prolonged disconnection) only achieves a service factor and energy use of about 85\%. % and the service factor in the optimized thresholds case is slightly less than that of the fixed threshold case, and both are close to 100\% which is much greater than that in the baseline. 
%We observe that the optimized and fixed threshold cases are able to provide more power to the refrigerator by reducing the use of the air compressor (Load A), which has the highest power demand and second highest energy use after the refrigerator. 
The air compressor (Load A) has a power demand that is much higher than other loads and the second highest energy demand. Although this load has the second highest priority, % and has the highest service factor in the baseline case. T
the optimized threshold case compromises serving this load to ensure better service to the higher priority Load D and the lower priority but lower energy demand Loads B and C. 
The baseline and fixed thresholds cases serve more energy to the air compressor, but have lower service factors for the microwave (Load C) and the washing machine (Load B).
%are third and fourth on the priority order respectively. These loads have the highest service factor in the optimized thresholds case. 
Because of this, the overall PSF in the optimized thresholds case is greater than that in the other two cases.  
Further, the optimized thresholds case and the baseline case fully use the allocated budget of 70\% of total desired energy, whereas the fixed thresholds case only uses 68\%. This is because the fixed thresholds case always has residual balance equal to at least the lowest threshold i.e. the threshold corresponding to the highest priority load.

% The power consumption by each load in the baseline case is shown in Figure \ref{fig:load_power_plot_case0}. It is seen that the customer experiences a disconnection from about Day 20 through Day 24. 

\begin{figure}%[htbp]
\centerline{\includegraphics[width = 0.67\columnwidth]{images/recharge70realrf5load_tsf_psf_barchart.pdf}}
\caption{\small Service factor for the 4 loads and overall priority service factor (PSF) at a recharge frequency of 5 per month and recharge amount of 70\%. Load priority: Load$\,$D$\,>\,$Load$\,$A$\,>\,$Load$\,$C$\,>\,$Load$\,$B}
\label{fig:recharge70realrf5load_tsf_psf_barchart}
\end{figure}

\begin{table}%[htbp]
\caption{Energy Usage per Load\vspace{-3mm}}
\begin{center}
\begin{tabular}{ll|l|l|l|l|l|l}%{m{2em} m{7em} m{3em} m{4em} m{3.5em}}
\hline
\multicolumn{2}{l|}{\multirow{3}{*}{\textbf{Appliance}}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Baseline}}} & \multicolumn{2}{c|}{\textbf{Fixed }} & \multicolumn{2}{c}{\textbf{Optimal}}\\
\multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{\textbf{ Thresholds}} & \multicolumn{2}{c}{\textbf{ Thresholds}}\\[+2pt]
%\hline
\multicolumn{2}{c|}{}  & \textbf{kWh} & \textbf{\%} & \textbf{kWh} & \textbf{\%} & \textbf{kWh} & \textbf{\%} \\ 
\hline
A & air compressor & 12 & 43 & 7.5 & 27 & 6.7 & 24 \\ 
B & washing machine  & 1.9 & 95 & 0.34 & 17 & 2.0 & 100 \\
C & microwave & 3.2 & 89 & 1.8 & 50 & 3.5 & 97 \\
D & refrigerator & 35 & 85 & 41 & 100 & 40 & 98 \\
\hline
\multicolumn{2}{l|}{\textbf{Total}} & 52.1 & 70 & 50.6 & 68 & 52.2 & 70\\
\hline
\end{tabular}
\vspace{-5mm}
\label{tab:energy-use-per-load}
\end{center}
\end{table}


% \begin{figure}%[htbp]
% \centerline{\includegraphics[width = \columnwidth]{images/load_power_plot_rechargefreq5rechargepercent70_case0.pdf}}
% \caption{Load power consumption in the baseline case (W).}
% \label{fig:load_power_plot_case0}
% \end{figure}


\subsection{Impact of Recharge Amount and Frequency}
Next, we compare the achieved PSF and the number of disconnections (i.e., how frequently the real wallet balance falls below zero and customers lose electricity supply) across different recharge amounts and frequencies.

\subsubsection{Impact on priority service factor}
The upper plot in Figure \ref{fig:priority_sf_plot} shows the variation in the PSF as the recharge amount is varied from 60\% to 100\% with a constant recharge frequency of 5 per month. The PSF increases with increasing recharge amount for all three cases, as expected. Across all recharge amounts, the optimized thresholds case has a PSF greater than the baseline while the fixed thresholds case performs worse due to the residual balance that remains unused. The bottom plot in Figure \ref{fig:priority_sf_plot} shows the variation in PSF as the recharge frequency is varied from 1 to 7 per month while keeping the recharge amount constant at 70\%. The optimized and fixed thresholds cases have minimal variation in PSF even if the recharge amount is distributed across increasing number of recharges during the month because the daily virtual wallet recharge remains the same. The optimized thresholds case performs better than the baseline whereas the fixed thresholds case performs worse due to the unused residual energy.

\begin{comment}
\begin{figure}%[htbp]
\centerline{\includegraphics[width = 0.4\textwidth]{images/realrf5priority_sf_plot.pdf}}
\caption{\small PSF against recharge amount at a recharge frequency of 5 per month. The optimized thresholds case performs better than the baseline whereas fixed thresholds performs worse. Increasing recharge amount increases priority service factor in each case.\vspace{-2mm}}
\label{fig:realrf5priority_sf_plot}
\end{figure}
\end{comment}

%\begin{figure}[htbp]
%\centerline{\includegraphics[width = 0.5\textwidth]{images/prepaid-chapter/realrf5energy_sf_plot.pdf}}
%\caption{Energy service factor against recharge amount at a recharge frequency of 5 per month for the %baseline, fixed, and optimized thresholds cases.}
%\label{fig:realrf5energy_sf_plot}
%\end{figure}

%\begin{figure}[htbp]
%\centerline{\includegraphics[width = 0.5\textwidth]{images/prepaid-chapter/realrf5load_tsf_barchart.pdf}}
%\caption{Service factor for the 4 loads at a recharge frequency of 5 per month and recharge amount of 60\% for the baseline, fixed, and optimized thresholds cases. Priority order of loads: Load 4 $>$ Load 1 $>$ Load 3 $>$ Load 2}
%\label{fig:realrf5load_tsf_barchart}
%\end{figure}




%%%

\begin{comment}
\begin{figure}%[htbp]
\centerline{\includegraphics[width = 0.4\textwidth]{images/recharge70priority_sf_plot.pdf}}
\caption{\small PSF against monthly recharge frequency at a recharge amount of 70\%. The optimized thresholds case performs better than the baseline whereas the fixed thresholds case performs worse.\vspace{-2mm}}
\label{fig:recharge70priority_sf_plot}
\end{figure}
\end{comment}

\begin{figure}%[htbp]
\centerline{\includegraphics[width = 0.45\textwidth]{images/realrf5recharge70priority_sf_plot.pdf}}
\caption{\small Top: PSF against recharge amount at a recharge frequency of 5 per month. %The optimized thresholds case performs better than the baseline whereas fixed thresholds performs worse. Increasing recharge amount increases priority service factor in each case. \\
Bottom: PSF against monthly recharge frequency at a recharge amount of 70\%. %The optimized thresholds case performs better than the baseline whereas the fixed thresholds case performs worse.
\vspace{-5mm}}
\label{fig:priority_sf_plot}
\end{figure}


%\begin{figure}[htbp]
%\centerline{\includegraphics[width = 0.5\textwidth]{images/prepaid-chapter/recharge70energy_sf_plot.pdf}}
%\caption{Energy service factor against monthly recharge frequency at a recharge amount of 70\% for the baseline, fixed, and optimized thresholds cases. The optimized thresholds case performs better than the baseline whereas fixed thresholds performs worse.}
%\label{fig:recharge70energy_sf_plot}
%end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Impact on disconnections}
We further investigate the impact of recharge frequency and amount on the number of disconnections. We first vary the recharge amount from 60\% to 100\% while keeping the recharge frequency constant at 5 per month, and then vary the recharge frequency from 1 to 7 per month while keeping the recharge amount constant at 70\%.
In all of these cases, both the fixed and optimized threshold cases result in zero disconnections as all loads were disabled before the real wallet balance could fall below zero. This demonstrates that the simple threshold-based management can avoid disconnections and associated reconnection fees.

This is quite an improvement relative to the baseline case. With 5 recharges per month, the baseline case experienced 3 disconnections for recharge amounts of 60\% and 70\% and one disconnection for recharge amounts $\geq 80$
\%.
When we fix the recharge amount at 70\%, we observe that the number of disconnections increase with increasing recharge frequency. With one recharge, we only have one disconnection, with 3 recharges we have 2 disconnections and with 5 and 7 recharges we have 3 disconnections. 
The reason for this behavior is that the recharge amounts are distributed uniformly across the month, whereas the load is not. For low recharge amounts or high recharge frequencies, there is therefore a higher chance that the real wallet balance might drop to zero before the next recharge is made whereas for higher recharge amounts and fewer payments, these intermediate disconnections are avoided. % and the only disconnection happens towards the end of the month. 

% Figure \ref{fig:realrf5disconnections_plot} shows the number of disconnections as the recharge amount is varied from 60\% to 100\% while keeping the recharge frequency constant at 5 per month. The fixed and optimized thresholds cases do not have any disconnections as expected. The number of disconnections in the baseline case decreases with increasing recharge amount since more funds are available to serve the demand. 
% Figure \ref{fig:recharge70disconnections_plot} shows the number of disconnections as the recharge frequency is varied from 1 to 7 per month while keeping the recharge amount constant at 70\%. The fixed and optimized thresholds cases do not have any disconnections. The number of disconnections in the baseline case increases with increasing recharge frequency because the recharge amount is distributed uniformly across each recharge in the month but the demand is not uniform as seen in Figure \ref{fig:load_power_plot}. Therefore, on days when the demand is higher there is a deficit in wallet balance causing a disconnection.

% \begin{figure}[htbp]
% \centerline{\includegraphics[width = 0.4\textwidth]{images/realrf5disconnections_plot.pdf}}
% \caption{\small Number of disconnections against recharge amount at a recharge frequency of 5 per month. No disconnections in the fixed and optimized thresholds cases. Disconnections decrease with increasing recharge amount in the baseline case.}
% \label{fig:realrf5disconnections_plot}
% \end{figure}



% \begin{figure}[htbp]
% \centerline{\includegraphics[width = 0.4\textwidth]{images/recharge70disconnections_plot.pdf}}
% \caption{\small Number of disconnections against monthly recharge frequency at a recharge amount of 70\%.  No disconnections in the fixed and optimized thresholds cases. Disconnections increase with increasing recharge frequency in the baseline case.\vspace{-5mm}}
% \label{fig:recharge70disconnections_plot}
% \end{figure}

==> Prepaid Electricity - IEEE PowerTech - arXiv/04-conclusions.tex <==
\vspace{-3mm}
\section{Conclusion}
\label{section:conclusion}
This work proposes a threshold-based energy rationing framework for prepaid customers. This framework compares a predetermined threshold with the prepaid wallet balance to decide whether a load can be used without impacting other, higher priority loads later. To determine the optimal threshold values, we formulate and solve a rolling horizon optimization problem.
% The framework has been presented in the context of LMI households in the United States and it can be extended for other contexts such as postpaid customers on energy assistance programs and pay-as-you-go solar home system users. 
The case study shows that the framework with optimized thresholds outperforms both a baseline without energy management and a method where control thresholds are fixed solely based on load priority information. Specifically, the proposed method serves higher priority loads and reduces disconnections by curtailing lower priority loads.

%We have assumed that perfect demand and recharge forecasts are available.
Some avenues for future work include studying the effects of imperfect forecasts of future demand and recharge frequency and amount. The effect of incorporating fixed and transaction costs can also be studied, and be used to inform overall prepaid program design. Finally, while the framework has been presented in the context of LMI households in the United States, it can be extended for other contexts such as postpaid customers on energy assistance programs and pay-as-you-go solar home system users. 
%It can also offer insights to users for scheduling recharges and help in effective budgeting of monthly expenses.

\begin{comment}
\begin{itemize}
    \item study effects of imperfect data on future demand, recharge frequency and amount
    \item incorporate a fixed cost component in addition to a variable \$/kWh rate
    \item incorporate transaction costs for each recharge
\end{itemize}
\end{comment}


